Attention-Based Planning with Active Perception

Attention control is a key cognitive ability for humans to select information relevant to the current task. This paper develops a computational model of attention and an algorithm for attention-based probabilistic planning in Markov decision processes. In attention-based planning, the robot decides to be in different attention modes. An attention mode corresponds to a subset of state variables monitored by the robot. By switching between different attention modes, the robot actively perceives task-relevant information to reduce the cost of information acquisition and processing, while achieving near-optimal task performance. Though planning with attention-based active perception inevitably introduces partial observations, a partially observable MDP formulation makes the problem computational expensive to solve. Instead, our proposed method employs a hierarchical planning framework in which the robot determines what to pay attention to and for how long the attention should be sustained before shifting to other information sources. During the attention sustaining phase, the robot carries out a sub-policy, computed from an abstraction of the original MDP given the current attention. We use an example where a robot is tasked to capture a set of intruders in a stochastic gridworld. The experimental results show that the proposed method enables information- and computation-efficient optimal planning in stochastic environments.

==> archive0330.tex <==

\normalcolor
\newpage


  \section{Analyzing the gap between a semi-optimal policy and the optimal policy}
  
  
\begin{definition}
\label{def:reward-preserving}
Given a state $x\in Dom(X)$ of \ac{mdp} $M$, an attention function $f$ is reward preserving for state $x$ if and only if  
\[
\bar{R}^f(f(x),a) = \ubar{R}^f(f(x),a), \quad \forall a\in \enabled(x)
\]
where $\enabled(x)$ is a set of actions enabled from state $x$.
\end{definition}
That is, the reward viewed by the optimistic agent and the pessimistic agent is the same, given a subset of states and an attention function. Let $\att: Dom(X)\rightarrow 2^\calF$ be the function that maps a state to a subset of reward-preserving attention functions. 
  
%   An action $a\in A$ is \emph{localized} with respect to a subvector $Y$ of vector $X$ 
%   if \[
% \forall x\in Dom(X), \quad  P(x'|x,a)= \prod_{X_i\in Y} P(x_i'| \parent(x_i), a) \cdot \prod_{X_j\notin Y}P(x_j\mid \parent(x_j)).\]
%   In this case, we say $a$ is $Y$-localized. In addition, an action $a$ is \emph{strongly $Y$-localized}  if 
%   \[
%   P(x'|x,a)= \prod_{X_i\in Y} P(x_i'| \parent(x_i), a)  
%   \]

%   \begin{assumption}
%   \label{assume:special-case}
%   The set of attention functions and the original \ac{mdp} satisfy
%   \begin{itemize}
%       \item For each state $x\in Dom(X)$, there exists an attention function $f$ that is reward preserving for $x$.
%       \item For each   action $a\in A$, there exists an attention function $f$ such that action $a$ is strongly $f(X)$-localized. 
%   \end{itemize}
%   \end{assumption}
%   Let $Act: \calF\rightarrow 2^A$ be a function that maps an attention function $f$ to a set of actions such that $a\in Act(f)$ only if $a$ is strongly localized with respect to $f$.
  
  \begin{definition}
 \label{def:attention-mdp}
  Given an \ac{mdp} $M$ and a set of attention function $f$, assuming ~\ref{assume:special-case}, a switching-attention \ac{mdp} $\cal M$ is defined by 
  \[
  {\cal M}= \langle Dom(X), \calF, \{G_f\}_{f\in \calF}, \inv \rangle 
  \]
  \begin{itemize}
      \item $Dom(X)$ is the set of states.
      \item $\calF$ is a set of discrete modes, defined by the attention function. Under each mode, the original \ac{mdp} is abstracted into an attention driven \ac{mdp}, defined 
$M^f= (Dom(f(X)), A, P^f)$.
      \item $G_f: Dom(f(X))  \rightarrow 2^{\calF}$ is the guard condition that maps a local state $y\in Dom(f(X))$ of \ac{mdp} $M^f$ into a subset of modes the system can switch to.
    \[
    G_f(y)=\{f' \mid \forall x'\in f^{-1}(y), f'\in \att(x') \}.
    \]
    
      \item $\inv: \calF \rightarrow 2^{Dom(X)}$ maps $f\in \calF$ to the invariant set, defined by 
      \[
      \inv(f) = \{x \in Dom(X)\mid f\in \att(x)\}.
      \]
  \end{itemize}
  \end{definition}
%   Intuition: This basically allows us to decompose the state space into subsets, for each subsets, there exists an subMDP that aggregates the original MDP. A different way to understand the attention function is that it is a state-aggregation function. By switching attention we allows the state to be aggregated in different ways, and at each time we select which aggregation it is to be applied.


\paragraph{Attention-selective control policies} Given an attention-driven \ac{mdp} $M^f$, a \emph{local, Markovian} control policy is a function $\pi^f: Dom(f(X))\rightarrow \dist(A)$ that maps an attended state to a distribution of actions. The set of local, Markovian policy given $M^f$ is denoted $\Pi^f$. We denote $\Pi^\calF = \cup_{f\in \calF}\Pi^f$. 

A  Markovian, deterministic, attention-switching policy in the \ac{mdp} ${\cal M}^\calF$ is a function $\pi$ that satisfies the following conditions: Given a pair $(y,f)$ of state in a local \ac{mdp} $M^f$, if $y\in Dom(G_f)$, then $\pi(y,f) = f'$ for some $f'\in G_f(y)$. Otherwise, the switching policy is undefined. A Markovian, stochastic, attention-switching policy $\pi$ maps a pair $(y,f)$ into a distribution of $\calF$ such that $\pi(f'| y,f) >0$ only if $f'\in G_f(y)$.

An optimal, Markovian policy in ${\cal M}^f$ is composed of $\pi^\ast$--a switching policy and $\{\pi^{f,\ast}, f\in \calF\}$--a set of local policies in attention-driven \ac{mdp}s. 


\subsection{MDP with parameterized actions} We consider a special case when the actions of the \ac{mdp} $M$ are parameterized: there is a finite set of discrete actions $Act= \{\alpha_1,\ldots, \alpha_k\}$, and each $\alpha \in Act$ has a set of random vector parameters $Y_\alpha \subseteq 2^X$.  A parameterized action is a tuple $(\alpha, y)$. The action space of the \ac{mdp} is given by 
\[
A = \cup_{\alpha_i \in Act} \{(\alpha, y)\mid y\in Y_\alpha\}.
\]

We say the set of parameterized actions are strongly localized, if the transition function satisfies
\[
P(x'|x, (\alpha, y)) = \prod_{x_k\in y} P(x_k'| \parent(x_k), (\alpha, y))
\]
Intuitively, by assignning a random vector to an action, the action will only affects the value of these random vector in the \ac{mdp}. The values of other random variables will remain unchanged.

\begin{lemma}
If the original \ac{mdp} has parameterized actions with localized effects, then there exists an optimal, deterministic, Markovian policy $\{\pi^\ast, \{\pi^{f,\ast}, f\in \calF\}\}$ that achieves the performance of the optimal policy in the original \ac{mdp} without switching attention. 
\end{lemma}
\begin{proof}
Constructive, we show the dynamic programming equation.
\end{proof}


\subsection{Attention-driven policies: The general case}

In the special case, the action has localized effect: If the agent pay attention to a subset of state variables, his parameterized actions only affects the values of these attended states. 
In this subsection, we consider the synthesis problem of optimal attention-driven policies in the general case.

We consider the selection of attention functions as ``high-level actions'' that affect the ``cognitive state'' of the planner. To incorporate the new action set and new states, we formulate an \ac{mdp} with augmented state and action space from Definition~\ref{def:attention-mdp}
\[
{\cal M} = \langle Dom(X)\times {\cal F}, A\cup {\cal F}, \calP, \beta, R\rangle
\]
where 
\begin{itemize}
    \item $Dom(X) \times {\calF }$ is a set of states.
    \item $A\cup {\calF}$ is a set of actions, including   MDP's actions and the set of  attention functions that can be selected.
    \item $\calP: Dom(X)\times \calF \times (A\cup \calF )\rightarrow D(Dom(X)\times \calF) $ is the probabilistic transition function, defined by 
    
\[
\calP ((x',f)\mid (x,f), a) = P(x'|x,a), \text{ for }a\in A, x\in \inv(f).
    \]
    \[
    \calP((x,f')\mid (x,f), f')=1,   \text{ for }f' \in G_f(f(x))
    \]
    otherwise, $\calP((x',f')|(x,f),z)=0$ for $z\in A\cup \calF$. 
    \item $\beta$ is the distribution over the initial state.
    \item $R:Dom(X)\times {\calF}\rightarrow \reals $ is the reward function, defined by $R((x,f),a)=r(x,a)$ for $a\in A$ and $R((x,f), f')=0$ for $f'\in \calF$.
\end{itemize}
In other words, at each history $h$, the agent can either take an action in the \ac{mdp}, or change the attention function.

In this \ac{mdp}, a deterministic, attention-driven policy $\pi: Dom(X)\times \calF\rightarrow \dist(A\cup \calF)$ satisfies the following constraint: $\pi(x, f) = \pi(x', f)$ for any $x, x'$ that $x\ne x'$ but $f(x)= f(x')$--that is, the two states have the same observation given the attention function. 


Given the augmented \ac{mdp} $\cal M$, two states $x_1,x_2$ are observation equivalent given the attention function $f$ if and only if $f(x_1)=f(x_2)$. Given a state $x\in Dom(X)$, let $[x]_f$ be the set of \emph{observation-equivalent} states w.r.t $f$. Next, we use principle of abstract DP to study planning problem with attention-switching \ac{mdp}.


\begin{definition}[Disaggregation probability function]
A disaggregation function $u: Dom(X)\times \calF\rightarrow \reals$ assigns each state $(x,f)$ a \emph{disaggregation probability} with respect to the equivalent class $[x]_f$. It holds that $\sum_{x_i\in [x]_f} u(x_i,f) =1$.
\end{definition}
The disaggragation probability $u(x_i,f)$ can be understood as the degree to which the aggregated state $[x]_f$ represents $x_i$. 


\begin{definition}[State-aggregation with attention functions] Given the original \ac{mdp} $M=(Dom(X), A, P)$ and the disaggregation function $u: Dom(X)\times \calF\rightarrow \reals$, for each attention function $f\in \calF$, there is a state-aggregated \ac{mdp} defined by
\[
\tilde M_f= \langle  \{[x]_f\mid x\in Dom(X)\}, A, \tilde P_f, \tilde R_f,\gamma \rangle 
\]
with the following components:
\begin{itemize}
    \item $  \{[x]_f\mid x\in Dom(X)\}$ is the set of abstract states, each abstract state includes a set of observation-equivalent states respecting  $f\in \calF$.
    \item $A$ is the  action set.
    \item $\tilde P_f$ is the abstract transition function, defined by  
    \[
    \tilde P_f(([x']_{f'} )\mid ([x]_f  ), a) = \sum_{x_i\in [x]_f} u(x_i,f)P(x_j\mid x_i, a)\mathbf{1}(x_j \in [x']_f)
    \]
     \item $\tilde R_f$ is defined by $\tilde R( [x]_f , a) = r(x,a)$ for any $x\in [x]_f$. This is because of the reward preserving property of attention function $f$.
\end{itemize}
\end{definition}

In this aggregated \ac{mdp}, we can formulate a  linear program to solve a Markovian, optimal and attention-driven policy $\pi^\ast$.

\paragraph*{Primal linear program}
\begin{align*}
    \min_{\tilde V_f} \quad  &  c^\top \tilde V_f\\
    \mbox{subject to:} \quad &
    \tilde V_f([x]_f ) \ge \tilde R_f([x]_f , a) + \Expect_{ \tilde P_f}\tilde V_f([x']_{f'} )
\end{align*}

The solution we in the aggregated \ac{mdp} is denoted $\tilde \pi_f$. Note that this policy depends on the disaggregation probability function $u$--that is, different disaggregation probability will yield different optimal policies in the aggregated \ac{mdp}. 

For an optimal policy in the aggregated \ac{mdp}, we can evaluate its performance in the original \ac{mdp} by policy evaluation step, which is to solve the following linear equation:
\[
V_f= R+\gamma P^{\tilde \pi_f}
V_f
\]where $V_f$ is the evaluation of the optimal policy obtained from $\tilde \cal M_f$ in the original \ac{mdp}.


Let $V$ denote the value of the optimal policy in the original \ac{mdp} with complete observation. Let's consider the disaggregation function is one of the design parameter. Then, the optimal attention-based policy should be the one that solve the following optimization problem: for each $f\in \calF$, 
\[
\min_{u} \norm{V_f -V}^2.
\]
where $V_f$ depends on $u$ incomplicitly. This problem can be solved for each $f$ individually because the function $u$ assigns independent probability distributions given different attention functions.

NOTE THAT finding the optimal disaggregation probability is not easy. We choose a uniform aggregation probability but divert to attention-switching to mitigate the suboptimality.

\subsection{Attention-switching policy}

For each optimal attention-based policy $\pi_f$, let $V_f: X\rightarrow \reals$ be the value of the policy in the original \ac{mdp}. In this section, we aim to answer: When to switch the attention? Which (set of variables) should we pay attention to?
 
  The important fact about attention is that a planner not only knows what it pays attention to, but also is conscious of what it does not pay attention to. Thus, given any history $h_t$ of past observation, the agent can determine a belief $b_t$ which consists of two part $(y_t, z_t )$ where $y_t$ is the fully observed states given the attention function at time $t$ and $Z_t$ is a probability distribution over values of unobserved state variables.

We propose an attention-switching policy: Let $f_t$ be the attention function at time $t$, and a belief $(y_t,z_t)$, the predicted future reward with the current attention function is 
\[
\Expect_{z_t \sim Z_t} V^{f_t}(y_t,z_t)
\]
In addition to the expected reward, we calculate the upper and lower bound on the future reward as 
\[
\overline{R}^{f_t} (y_t,Z_t ) = \max_{z_t \in \supp( Z_t)} V^{f_t}(y_t,z_t),
\]
and 
\[
\underline{R}^{f_t} (y_t,Z_t ) =\min_{z_t \in \supp( Z_t)} V^{f_t}(y_t,z_t).
\]
When $
\overline{R}^{f_t} (y_t,Z_t )  - 
\underline{R}^{f_t} (y_t,Z_t ) \ge \epsilon$ where $\epsilon >0$ is a pre-defined threshold, the agent needs to re-select an attention function that minimizes the following quantity: The entropy in the current belief. This is called the \emph{belief refinement step}. Once the belief is refined so that the  $
\overline{R}^{f_t} (y_t,Z_t )  - 
\underline{R}^{f_t} (y_t,Z_t ) < \epsilon$, then the agent will select an attention function that maximizes the expected future reward.

\begin{lemma}
Conjecture: The value of the proposed online attention-switching policy should outperform any fixed attention-based policy.
\end{lemma}

\begin{lemma}
Conjecture: 
The value of the proposed online policy given the initial state should be $g(\epsilon, \eta)$-close to the optimal policy that uses full attention. here $\epsilon$ is the bound in determining when to select attention, and $\eta$ is the bound on the performance evaluation for an attention switching policy. $\eta = \max_s \min_{f}(V^f(s) - V(s))$ and a guess of this function $g(\epsilon,\eta) = \epsilon+\eta$.
\end{lemma}


\begin{lemma}
Conjecture:

relate to semi-optimal value function. 

\end{lemma}


\newpage

==> archive1.tex <==
% some notes relates the value functions of two different MDPs.
% \begin{comment}
To relate the optimal policy $\pi^\ast$ in $\tilde {\cal M}$ in the original \ac{mdp}, we denote $V:Dom(X)\times \calF\rightarrow \reals$ to be the evaluation of policy $\pi^\ast$ in the attention-switching \ac{mdp} $\calM$. 

\begin{lemma}Assuming that the policy $\pi^\ast$-induced chain is ergodic, there exists a weight function $u$ such that $ \tilde V([x]_{f},f) =\sum_{x_i\in [x]_f}u(x_i,f)V(x_i,f)$.
\end{lemma}
\begin{proof}
The value of the optimal policy in $\tilde {\cal M}$ satisfies the Bellman equation
\[
   \tilde V([x]_f,f) = \Expect_{a\sim \pi^\ast([x]_f,f)} 
   \left[\tilde R(([x]_f,f),a) + \sum_{x_i\in [x]_f} u(x_i, f)\sum_{x_j} P(x_j\mid x_i, a) \tilde{V} ( [x_j]_f ,f)
   \right]
   \]
   substituting the value function $ \tilde V([x]_{f},f) =\sum_{x_i\in [x]_f}u(x_i,f)V(x_i,f)$, we have
   \[\sum_{x_i\in [x]_f}u(x_i,f)V(x_i,f) = \Expect_{a\sim \pi^\ast([x]_f,f)} 
   \left[\tilde R(([x]_f,f),a) + \sum_{x_i\in [x]_f} u(x_i, f)\sum_{x_j} P(x_j\mid x_i, a) \left(\sum_{x_k\in [x_j]_f}u(x_k,f)V(x_k,f)
   \right) \right]
   \]
   on the other hand, from policy evaluation given the \ac{mdp} $\cal M$, we have 
   
\[  V(x_i,f) = \Expect_{a\sim \pi^\ast([x]_f,f)} \left[R(x_i,f),a) +  \sum_{x_j} P(x_j\mid x_i, a) V( x_j ,f)\right]
\]
multiply each side by $u(x_i,f)$ and sum over all $x_i\in [x]_f$, 
we have 
\[\sum_{x_i\in [x]_f}u(x_i,f)V(x_i,f)= \Expect_{a\sim \pi^\ast([x]_f,f)} \left[\sum_{x_i\in [x]_f}u(x_i,f) R(x_i,f),a) +  \sum_{x_i\in [x]_f}u(x_i,f) \sum_{x_j} P(x_j\mid x_i, a) V( x_j ,f)\right]
\]
equating the right-hand-side of two equations, we have 
\begin{align*} \Expect_{a\sim \pi^\ast([x]_f,f)} 
   \left[\tilde R(([x]_f,f),a) + \sum_{x_i\in [x]_f} u(x_i, f)\sum_{x_j} P(x_j\mid x_i, a) \sum_{x_k\in [x_j]_f}u(x_k,f)V(x_k,f)
   \right]\\
    = \Expect_{a\sim \pi^\ast([x]_f,f)} \left[\sum_{x_i\in [x]_f}u(x_i,f) R((x_i,f),a) +  \sum_{x_i\in [x]_f}u(x_i,f) \sum_{x_j} P(x_j\mid x_i, a) V( x_j ,f)\right]
\end{align*}
which implies,  
\[  \sum_{x_k\in [x_j]_f}u(x_k,f)V(x_k,f)
=  V( x_j ,f), \forall j
\]
This is because $\sum_{x_i\in [x]_f}u(x_i,f)=1$ and $R((x_i,f),a) = R(([x]_f,f),a)$ due to the reward preserving property of the attention function. 
 \textcolor{wrong!}
 
 We have $(I- U)V = 0$. If such a $U$ mat exists. then this should be the weight. 
\end{proof}
%\end{comment}


\paragraph*{LP }
Let $\nu(f,a) $ be the fraction of time of reaching a mode $f$ and taking the action $a$.  Let $\mu((x,f),a)$ be the fraction of time of reaching the state $(x,f)$ and taking the action $a$. (We assume the absorbing case.) The objective function is given by 
\[
\max_{\mu, \nu}\sum_{(x,f), a} \mu((x,f),a) R((x,f),a)
\]
and the constraints are

\[
\sum_{a\in A}\mu((x,f),a) =\beta(x,f)+ \sum_{(x',f')}\nv(f,a) P((x,f)| (x',f'), a)
\]
and 
\[
\sum_{x \in \inv(f)} \mu((x,f),a) = \nu(f,a).
\]
where $\beta$ is the initial distribution. 

% \begin{lemma}
% Given the null attention function, the solutions of optimistic planner and pessimistic planner are the same  $(\bar{V}^{f_0} =\ubar{V}^{f_0}= V^{f_0}, \bar{\pi}^{f_0} =\ubar{\pi}^{f_0}= \pi^{f_0})$. Further, for any other $f\in \calF$, it holds that 
% \[
% \bar{V}^f \ge V^{f_0} \ge \ubar{V}^f 
% \]
% where $\ge$ is element-wise comparison of vectors of values.
% \end{lemma}


% In the \ac{mdp} $\cal M$, given a history $\rho =(x_0,f_0)(x_1, f_1)\ldots (x_n, f_n)$, the observation is given by $\hat \rho = f_{0}(x_0)f_{1}(x_1)\ldots f_{n}(x_n)$. An \emph{admissible} policy $\pi$ maps the observation $\hat \rho $ into a distribution over $A\cup \calF$. 
% Note that the difference between POMDP and attention-driven \ac{mdp} is that in POMDP, the agent maintains a belief of the current state, as a probability distribution. In the attention-driven \ac{mdp}, the agent each time only is to solve the optimal policy in the MDP with complete observation of variables he pays attention to.

% Fact 1:  Given the total discounted reward maximization problem, the optimal policy $\pi^\ast $ in $\cal M$ reduces to the optimal policy in the original \ac{mdp} $M$ as the planner will select the null attention function to monitor all state variables at every step.

% Our question is, how to incorporate the benefit of using an incomplete attention function as a reward function?


% \subsection{Special case}

% We consider the following question: Suppose the null attention function is not available for the agent, under which condition can the optimal \emph{attention-switching} policy achieves the same performance as the optimal policy in the original \ac{mdp}? 

% To answer this question, let's first introduce the notion of sub-MDP \cite{}. 

% Given an \ac{mdp} $M$,  a subMDP of $M$ is defined by a pair $ (C,D)$ where $C$ is a subset of states, and $D:C\rightarrow 2^A$ is a function that maps a state $s\in Dom(X)$ to a set of \emph{enabled} actions such that $a\in D(x)$ only if $supp(P(\cdot | s,a)) \subseteq C$. That is, when an enabled action is taken, then the agent only reaches a state in the sub-MDP with a nonzero probability.



% \subsection{The option framework for planning with selective attention}
% We now construct an MDP that only allows attention-selective actions.


% \begin{definition} Given an attention-driven \ac{mdp} $M^f = \langle Dom(Y), A, P^f, y_0 \rangle$, an  \emph{attention-driven    option} $ o^f$ is a tuple 
% \[
%  o^f = \langle \pi^{f}, \beta^f, I^f\rangle,
% \]
% where $\pi^{  f}: Dom(Y)\rightarrow \dist(A) $ is a    policy in $M^f$. $\beta^f: Dom(Y)\rightarrow [0,1]$ is a termination function: given  a state $y\in Dom(Y)$, $\beta^f(y)$ is the probability of terminating the policy at that state. $I^f$ is a set of states from which this policy can be initiated.
% \end{definition}
\begin{comment}
\begin{definition}[Attention-selective MDP]
Given an \ac{mdp}  $M= (  Dom(X), A,P, x_0, R)$ and a set ${\cal F} = \{f_1,\ldots, f_m\}$  of attention functions, the \emph{attention-selective \ac{mdp}} is a tuple
\[
{\cal M} = \langle Dom(X) \times \calF,  \calF, P, (x_0, f_0), R\rangle
\]
with the following components:
\begin{itemize}
    \item $Dom(X)\times \calF$ is the set of state space.
    \item $\options = \cup_{f\in \calF}\{\bar{o}^f, \ubar{o}^f\}$ is a set of attention-driven options. $\bar o^f  = \langle \bar{\pi}^{\ast, f} , \bar{\beta}^f , \bar{I}^f  \rangle $ is an option based on the optimistic policy.  $\ubar{o}^f  = \langle \ubar{\pi}^{\ast, f} , \ubar{\beta}^f , \ubar{I}^f \rangle $  is an option based on the pessimistic policy.
    \item $P: Dom(X)\times \options\rightarrow Dom(X)$ is the transition function:
    \[
    P(x'|x, o) = \sum_{k=1}^\infty p(x'
,k)\gamma^k\]
where $\gamma$ is the discounting factor, and $p(x', k)$ is the probability of terminating the option $o\in \options$ in exactly $k$ steps at the state $x'$.
\item $R: Dom(X)\times \options \rightarrow \reals$ is the reward function
\[
R(x,o) = \Expect\left\{\sum_{k=1}^\infty p(k)\left\{\sum_{t=0}^k (\gamma^t R(x_t, a_t))
\right\}\mid x_0=x\right\}
\]
where $p_k$ is the probability of terminating the option in $k$ steps.
\end{itemize}

\end{definition}
 The optimal policy in $\cal M$, denoted $\pi^{\ast}_o$ is a policy that achieves the value function $V^\ast_o$ that satisfies the Bellman equation. The optimal policy in $M_o$ is called \emph{semi-optimal} in the original \ac{mdp} $M$. 
 
  Next, we aim to answer: under which condition the optimal policy in the attention-selective \ac{mdp} is indeed optimal in the original \ac{mdp}.
  


  \begin{lemma}
  The optimal policy in the attention-selective \ac{mdp} with self-aware options only is also optimal in the original \ac{mdp} if 
       for each state $x\in Dom(X)$ for which $f$ is reward-preserving, for each action $a\in A$ enabled from $x$, $a$ is strongly $f(X)$-localized.
  \end{lemma}

\begin{proof}
[Sketch]
The semi-optimal policy satisfies 
\[
V_o(x)= R(x,\pi_o(x))+ \sum_{x'} P(x'|x, \pi_o(x)) V_o(x')  
=  \Expect\left\{\sum_{k=1}^\infty p(k)\left\{\sum_{t=0}^k (\gamma^t R(x_t, a_t))
\right\}\mid x_0=x\right\}+  \sum_{k=1}^\infty p(x'
,k)\gamma^k
\]
When the option is self-aware, 
\end{proof}
\end{comment}
